Predicting infections in the Covid-19 pandemic -- lessons learned

Throughout the Covid-19 pandemic, a significant amount of effort had been put into developing techniques that predict the number of infections under various assumptions about the public policy and non-pharmaceutical interventions. While both the available data and the sophistication of the AI models and available computing power exceed what was available in previous years, the overall success of prediction approaches was very limited. In this paper, we start from prediction algorithms proposed for XPrize Pandemic Response Challenge and consider several directions that might allow their improvement. Then, we investigate their performance over medium-term predictions extending over several months. We find that augmenting the algorithms with additional information about the culture of the modeled region, incorporating traditional compartmental models and up-to-date deep learning architectures can improve the performance for short term predictions, the accuracy of medium-term predictions is still very low and a significant amount of future research is needed to make such models a reliable component of a public policy toolbox.

==> NotIncluded.tex <==

PANDEMIC RESPONSE CHALLENGE

----

Draft of new intro: 

After 18 months of the spread of the COVID pandemic, we can safely say that humanity had shown remarkable progress on the development of diagnostics tools, vaccines and medications for the viral infection, our ability to predict the evolution of the pandemic had been very limited. Predicted increases in the number of infections did not materialize, on the other hand, significant spikes happened when the medical and political consensus predicted a return to normal. Such prediction errors occurred not only in the initial phases of the pandemic, but also after many months. Even if the COVID-19 pandemic ends up under control by the end of 2021, our inability to predict the evolution of the pandemic even 18 months into it, does not bode well for future health emergencies. 

This paper describes the approaches our team took when participating in the XPrize Pandemic prediction competition which regularly scored in the top 5-10 teams in the daily ledger(?) and qualified to the final of the competition which focused on prescriptive measures.

%%%%%% we can add this here as a footnote.

% ~\footnote{PAndemic Wave Predictor (PaWP) team , United States, https://www.xprize.org/challenge/pandemicresponse/articles/pandemic-response-challenge-finalists}.

We felt, however, that the prediction problem remains unsolved. Thus we also describe a number of improvements we added to our algorithms since the competition. We have also learned from the successive evolution of the pandemic. The approaches we describe take into consideration the cultural factors in the spread of the pandemic, and investigate the use of cutting edge machine learning models (deep neural networks using the Transformer pattern for sequence prediction). 

In addition to the lessons learned during the competition, we also describe several extensions we developed since 

--- 

Our approach is based on the recognition that the spread of the pandemic cannot be successfully predicted with a purely black box computational model. First of all, interpretability is important, especially for models that might drive public policy. But, second, the raw learning data is simply not sufficient for learning models of the type typically used in ``big data'' type of scenarios. For the predictions to be successful, the available data needs to be complemented with knowledge encoded in a more structured form. Thus, our model aims to use existing knowledge from epidemiology, sociology, cultural models and geography, in additional to machine learning and deep neural networks.

First of all, we need to take advantage of the established models, such as the compartmental models of epidemiology. These models capture in a simplified formal form significant experience about how diseases spread in a population. At the same time, some of the assumptions underlying these models were not upheld during the COVID-19 outbreak. This epidemic had dominated the public discourse in several countries, which triggered changes of the behavior of the population several times during the pandemic. These changes had been usually triggered by changes in the infected population, creating a delayed feedback loop. For instance, changes in the local ordinances (lock down, mask wearing mandates, opening / closing of schools and businesses, encouraging / discouraging tourism and travel) and recently, the distribution and administration rate of vaccines introduce variations that cannot be captured by epidemiological model alone. 

This led us to consider factors that are social and cultural in nature. Some of these had been extensively discussed in the last months, but rarely quantified explicitly. For instance, it was hypothesized that the individualistic nature of the American culture led to a lower compliance with mask wearing mandates, affecting the infection rate. However, the study of the numbers show that these aspects can be at best a partial explanation, which would not explain the significant differences  between the United Kingdom and Australia. Another consideration worth taking into account is geographical proximity, but this does not explain the differences between different nations of Scandinavia which are close both geographically and culturally. It turns out that public policy and discourse differences might be also driven by influential individuals, such as political, scientific or religious leaders. Such aspects are very hard to predict. 

In conclusion, our prediction and intervention plan models are based on the insight that the prediction is by augmenting the established epidemiological models with techniques that take into account the various factors that cause their parameters to change rapidly during the outbreak. Our proposition is to learn the way in which these parameters change using deep learning techniques that take into account features dependent on social, cultural and geographical aspects. We conjecture that these features have influences with complex inter-dependencies, but they can be learned by state of the art deep neural network models.


Our contributions in this paper are as follows: 
\begin{itemize}
    \item We study different prediction approaches to predict the number of new cases based on the history of data for each country. We studied lstm network LSTM Hofstede SIR, lstm xprize, and Transformer Hofstede SIR and compared them for all of the regions and for each country separately.  

\end{itemize}

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************

